Scalable Variational Bayes Inference for Dynamic Variable Selection

We develop a variational Bayes approach for dynamic variable selection in high-dimensional regression models with time-varying parameters and predictors that exhibit a predefined group structure. Through comprehensive simulation studies, we demonstrate that our method yields more accurate parameter estimates than existing Bayesian static and dynamic variable selection approaches while maintaining computational efficiency. We illustrate the performance of our approach within the context of a popular problem in economics: forecasting inflation based on a large set of macroeconomic predictors. Our approach demonstrates significant improvements in out-of-sample point and density forecasting accuracy. A retrospective analysis of the time-varying parameter estimates reveals economically interpretable patterns in inflation dynamics.

==> Tables/MSE_equity.tex <==
\begin{table}[htbp]
  \centering
 \renewcommand{\arraystretch}{0.6}
\resizebox{1\textwidth}{!}{   \begin{tabular}{lrrrrrrrrrrrr}
\toprule
          & \multicolumn{1}{l}{{\tt cOLS}} & \multicolumn{1}{l}{{\tt cPred}} & \multicolumn{1}{l}{{\tt HS}} & \multicolumn{1}{l}{{\tt F1}} & \multicolumn{1}{l}{{\tt EMVS}} & \multicolumn{1}{l}{{\tt GLP}} & \multicolumn{1}{l}{{\tt BGS}} & \multicolumn{1}{l}{{\tt BG group}} & \multicolumn{1}{l}{{\tt BGH}} & \multicolumn{1}{l}{{\tt DSS(5)}} & \multicolumn{1}{l}{{\tt DSS(9)}} & \multicolumn{1}{l}{{\tt DVS}} \\
          \midrule 
       RMSE   & \cellcolor[rgb]{ .988,  .945,  .957}1.000 & \cellcolor[rgb]{ .988,  .949,  .957}1.000 & \cellcolor[rgb]{ .988,  .875,  .886}1.010 & \cellcolor[rgb]{ .988,  .941,  .953}1.001 & \cellcolor[rgb]{ .988,  .878,  .89}1.010 & \cellcolor[rgb]{ .988,  .878,  .886}1.010 & \cellcolor[rgb]{ .988,  .988,  1}0.994 & \cellcolor[rgb]{ .988,  .949,  .961}1.000 & \cellcolor[rgb]{ .988,  .914,  .922}1.005 & \cellcolor[rgb]{ .984,  .733,  .741}1.030 & \cellcolor[rgb]{ .984,  .71,  .718}1.033 & \cellcolor[rgb]{ .973,  .412,  .42}1.074 \\
       \midrule
    $LS$ & \cellcolor[rgb]{ .973,  .529,  .537}-7.459 & \cellcolor[rgb]{ .984,  .984,  .996}0.001 & \cellcolor[rgb]{ .984,  .984,  .996}-0.005 & \cellcolor[rgb]{ .984,  .984,  .996}-0.004 & \cellcolor[rgb]{ .984,  .98,  .992}-0.021 & \cellcolor[rgb]{ .98,  .698,  .71}-4.637 & \cellcolor[rgb]{ .988,  .988,  1}0.054 & \cellcolor[rgb]{ .984,  .984,  .996}0.023 & \cellcolor[rgb]{ .984,  .984,  .996}-0.008 & \cellcolor[rgb]{ .984,  .976,  .988}-0.125 & \cellcolor[rgb]{ .984,  .976,  .988}-0.129 & \cellcolor[rgb]{ .973,  .412,  .42}-9.391 \\
    \bottomrule
    \end{tabular}}
\caption{\small This table reports the out-of-sample root mean squared prediction error and log-predictive score across models. The sample period is from 1971M1 to 2021M12. The first prediction is generated in 1991M11.}    
  \label{tab:mse_equity}%
\end{table}%

